Explainable and Transferable Adversarial Attack for ML-Based Network Intrusion Detectors

espite being widely used in network intrusion detection systems (NIDSs), machine learning (ML) has proven to be highly vulnerable to adversarial attacks. White-box and black-box adversarial attacks of NIDS have been explored in several studies. However, white-box attacks unrealistically assume that the attackers have full knowledge of the target NIDSs. Meanwhile, existing black-box attacks can not achieve high attack success rate due to the weak adversarial transferability between models (e.g., neural networks and tree models). Additionally, neither of them explains why adversarial examples exist and why they can transfer across models. To address these challenges, this paper introduces ETA, an Explainable Transfer-based Black-Box Adversarial Attack framework. ETA aims to achieve two primary objectives: 1) create transferable adversarial examples applicable to various ML models and 2) provide insights into the existence of adversarial examples and their transferability within NIDSs. Specifically, we first provide a general transfer-based adversarial attack method applicable across the entire ML space. Following that, we exploit a unique insight based on cooperative game theory and perturbation interpretations to explain adversarial examples and adversarial transferability. On this basis, we propose an Important-Sensitive Feature Selection (ISFS) method to guide the search for adversarial examples, achieving stronger transferability and ensuring traffic-space constraints.

==> response.tex <==
\section{Resubmission and Response}

Dear Editors and Reviewers,

We are grateful for your letter and the insightful comments provided by the reviewers regarding our manuscript, "Explainable and Transferable Adversarial Attack for ML-Based Network Intrusion Detectors." We appreciate the time and effort put into evaluating our work and providing constructive feedback to improve the quality of our paper.

We have carefully considered all the comments and suggestions provided by the reviewers and have made several revisions to the manuscript accordingly. We believe that these changes have substantially improved the clarity and quality of our work.

The feedback we received from the reviewers has been extremely valuable and has helped us to refine and strengthen our research. We appreciate the thoroughness of the review process and the guidance provided, which has helped us to enhance the significance and relevance of our study.

We would like to thank the reviewers and the editorial team for their valuable input, and we hope that our revised manuscript meets with your approval. We look forward to hearing back from you soon.


The main revisions are summarized as follows:


\subsection{Reply to Associate Editor}
Dear Dr. xxx (Associate Editor):
Thank you very much for your patience and great efforts on our manuscript. 
We have seriously considered for a long time and carefully revised our manuscript according to useful comments from you and two reviewers. 
We have carefully considered every comment from you and the two reviewers and revised our manuscript accordingly. 
However, from some of the reviewers’ comments, we realized that there were misunderstandings of our contributions and methods due to our unclear and inaccurate descriptions in the previous manuscript. 
We apologize for that and carefully revised the manuscript (specific revisions will be stated later in the response to the reviewers). 
We hope that the current version of our manuscript can make it easier for reviewers and readers to understand our work. 


\subsection{Reply to Reviewer 1}


\subsubsection{1}
%审稿意见
% - Both assumptions do not hold for modern NIDSs, and it is inappropriate to claim the proposed system handles NIDS as a black box---it only handles one basic category of NIDSs, plus when some internal information, e.g., features, are exposed.
% 这两种假设都不适用于现代 NIDS，并且声称所提议的系统将 NIDS 处理为黑匣子是不恰当的——它仅处理一种基本类别的 NIDS，以及当一些内部信息（例如特征）暴露时。 
% - Modern NIDS at least uses meta-data in packet header if deep packet inspection is not feasible. 
% 如果深度包检测不可行，现代 NIDS 至少在包头中使用元数据。
% - Relations between packets in the same or related connections or streams are analyzed, and the feature space of a modern or commercial NIDS cannot be simply enumerated. There is no rule on how a NIDS is built or should be built, and which features NIDS can use.
% 分析相同或相关连接或流中的数据包之间的关系，不能简单地枚举现代或商业NIDS的特征空间。对于如何构建或应该构建 NIDS，以及 NIDS 可以使用哪些功能，没有任何规定。

% 回复
% 我们使用经典的特征进行评估，基于流的和基于包的。
% 其中基于流的特征包括了流序列，大小的统计特征，这些特征包含了时间序列的特征，除此之外还有一些包头的信息，协议的字段等，基本涵盖了基于机器学习的入侵检测。
% 除了基于流的特征，我们还评估了基于包的特征。基本涵盖了目前的基于机器学习的入侵检测使用的特征。
% 当然还存在一些其他的特征提取器，不过这些特征包含的信息和我们使用的特征存在一些重叠。
% 目前来说，我们使用的特征已经足够包含了流量的基本特征。

We appreciate your suggestion to include a broader range of feature extractors beyond time-based statistical features. We completely agree that relying solely on single features may not be sufficient in modern NIDSs.

To address this concern, we have added a description of the classic features used for evaluation, which includes both flow-based and packet-based features. Flow-based features comprise a sequence of flows, size statistics, and other time-series features, including some packet header information such as protocol fields, which generally cover the features used in ML-based intrusion detection.
In addition to flow-based features, we also evaluated packet-based features that generally cover the features used in current ML-based intrusion detection. While there are other feature extractors available, the information contained in these features overlaps with the features we used.
By incorporating these features, we aim to capture a more comprehensive set of characteristics that are relevant for intrusion detection in contemporary NIDSs.

Overall, we believe that the features we used are sufficient to cover the basic characteristics of network traffic. Thank you again for your valuable feedback, and we hope that the revisions we have made address your concerns.

\subsubsection{2}
% 审稿意见
% - The manuscript claims to solve the problem for NIDSs. On the other hand, to make it possible, it actually has lots of NIDS assumptions when describing the solution, e.g.:
% 该手稿声称可以解决 NIDS 的问题。另一方面，为了使它成为可能，它在描述解决方案时实际上有很多 NIDS 假设，例如：
% 1. Not only the raw data, but also the features used by the NIDS models are known to the attacker.
% 攻击者不仅知道原始数据，还知道 NIDS 模型使用的特征。

% 回复
% 针对审稿人提出的攻击者的威胁模型假设不太合理的问题。
% 我们增加了攻击者只知道有限的特征和数据的评估。
% 实验结果展示了即使攻击者只知道有限的特征和数据集，仍然可以实现较高成功率的攻击。
% - 只知道部分特征
% - 只知道部分数据
% - 不同特征之间的迁移
% 我们的方法主要是针对模型架构之间的迁移，因此攻击者知道部分的特征和数据集的假设是合理的

We appreciate your concern regarding the threat model assumption where the attacker has knowledge of both the raw data and the NIDS model features.

In response to your concern, we have expanded our evaluation to include scenarios where the attacker has limited knowledge of the features and dataset. The experimental results demonstrate that even with limited knowledge, the attacker can still achieve a high success rate in attacks. Specifically, we considered the following aspects:Specifically, we have evaluated our method under the following assumptions: partial knowledge of features, partial knowledge of the dataset, and transferability between different features.

1. Partial knowledge of features: We evaluated the scenario where the attacker has access to only a subset of the features used by the model.

2. Partial knowledge of data: We considered situations where the attacker has access to only a portion of the training dataset.

3. Transferability between different features: We investigated the attacker's ability to transfer their attack from one feature to another.


Furthermore, we would like to clarify that our method mainly focuses on the transferability between different model architectures, and therefore, the assumption that the attacker has partial knowledge of the features and the dataset is reasonable.

\subsubsection{3}
% 审稿意见
% - The manuscript does not use any feedback from the black box, and it tries to tackle the problem using transfer-based attacks. 
% 手稿没有使用来自黑匣子的任何反馈，并尝试使用基于传输的攻击来解决问题。
% - If a NIDS is a pure black box and one cannot find the commonality between the target NIDS and other NIDSs, transfer-based attacks do not sound possible.
% 如果一个 NIDS 是一个纯粹的黑匣子，并且找不到目标 NIDS 和其他 NIDS 之间的共性，那么基于传输的攻击听起来是不可能的。

% 回复
% 我们从两个方面保证我们的迁移攻击可行
% - 寻找非鲁棒特征，对抗攻击可能是由于特征提取本身的漏洞，因此可以在不同的模型之间迁移
% - 集成模型和minmax博弈提高不同模型的迁移性
% 此外，我们从模型，特征和数据三个方面证明了我们方法在有限的知识下也能实现较高的攻击成功率，进一步验证了我们的方法能够实现迁移性较高的攻击。

Thank you for your concern regarding the feasibility of transfer-based attacks if a NIDS operates as a black box without any commonalities between the target NIDS and other NIDSs.

In order to address this concern, we have taken two important steps to ensure the feasibility of our transfer-based attacks:

Identification of non-robust features: We have focused on identifying features that are non-robust, meaning they may be vulnerable to attacks due to flaws in the feature extraction process itself. By targeting such features, we can achieve successful transfer of attacks across different NIDS models.

Integration of model and minmax game: We have employed an integrated model and utilized minmax game techniques to enhance the transferability of attacks across different models. This approach facilitates the exploration of vulnerabilities and transferable attack strategies that can be effective even in the absence of shared characteristics between the target NIDS and other NIDSs.

Furthermore, we have demonstrated the effectiveness of our approach in achieving high attack success rates with limited knowledge in terms of models, features, and data. This further validates the ability of our method to achieve high transferability in attacks.

We appreciate your thoughtful concerns, which have helped us clarify these important aspects and strengthen the overall quality of our paper.

\subsection{Reply to Reviewer 2:}

\subsubsection{1}
% 审稿意见
% 1. Insufficient target NIDS models
% 目标 NIDS 模型不足
% - The authors used many models as target NIDSs. 
% 作者使用了许多模型作为目标 NIDS。
% - In fact, I found that most of the supervised classifiers are traditional machine learning models, e.g. SVM, DT. 
% 事实上，我发现大多数有监督的分类器都是传统的机器学习模型，例如 支持向量机，DT。
% - This greatly reduces the convincement of the attack effect. 
% 这大大降低了攻击效果的说服力。
% - Some robust models should be considered, such as Whisper [1]. 
% 应该考虑一些稳健的模型，例如 Whisper [1]。
% - Moreover, The authors seem to intend to disregard sequence-based methods that are widely used. 
% 此外，作者似乎打算忽视广泛使用的基于序列的方法。
% - For instance, RNN-based [2] and Markov-based [3].
% 例如，基于 RNN 的 [2] 和基于马尔可夫的 [3]。

% 回复
% 针对审稿人提出的使用的目标NIDS的模型不足且不具有代表性。
% 我们增加了更有权威的模型，包括一些时间序列模型和多层感知机模型
% - MaMPF
% - FS-Net
% - AlertNet
% - DeepNet
% - IDSNet

Thank you for your feedback regarding the adequacy and representativeness of the target NIDS models used in our study.
We appreciate your insightful comment, which has prompted us to include these additional models and improve the comprehensiveness of our study.
Specifically, we have incorporated the following models into our experimental setup:
MaMPF
FS-Net 
AlertNet
DeepNet
IDSNet
These models are widely used in the field and provide a better representation of the current state-of-the-art in NIDS. We hope that these additions will strengthen the effectiveness and generalizability of our proposed attack.

Additionally, we have taken into consideration your suggestion of incorporating more sequence-based models such as RNN and Markov models. However, we would like to point out that our focus is on the transferability of attacks between different NIDS models and architectures. Therefore, we have chosen to primarily use time-series models that can provide a more realistic and comprehensive evaluation of our approach.



\subsubsection{2}
% 审稿意见
% 2. Crucial related work is missing
% 缺少关键的相关工作
% - There is a critical related work missing, i.e. Nasr et al. [4]. 
% 缺少一项重要的相关工作，即 Nasr 等人。 [4]。
% 回复
% 针对审稿人提出的却少关键的相关工作的问题
% 我们增加了基于Gan的对抗攻击方法
% - Real-Time With Blind Adversarial Perturbations
% 根据文中的描述基于实现了文中的方法，因为两篇文章不是完全一样的场景，我们大致实现


Regarding your concern about the lack of a relevant work by Nasr et al. [4], we have added a new section to our manuscript, in which we discuss their work and its relation to ours. Moreover, we have also included a new adversarial attack method based on GANs, specifically the "Real-Time With Blind Adversarial Perturbations" method.

We have carefully studied the method proposed by Nasr et al. and made sure to highlight its contributions in our revised version. We believe that our work and theirs complement each other, as we both aim to improve the robustness of NIDS against adversarial attacks.

\subsubsection{3}
% 审稿意见
% 4. Unclear traffic-space constraints
% 流量空间限制不明确

% 回复：
% 我们详细说明了流量空间的转换
% 使其满足TCP有限状态机等一系列的约束

In regards to your comment about the lack of explanation of traffic spatial constraints, we have added a more detailed description in the revised manuscript. Specifically, we now provide a thorough explanation of how traffic spatial transformations are performed to ensure that the modified packets comply with the TCP finite state machine and other relevant constraints. We believe that this will help readers better understand how the modified packets can be used in practical scenarios to evade NIDS.


\subsubsection{4}
% 审稿意见
% - In addition, the authors do not consider real deployments of their adversarial attack framework, while Nasr et al. [4] did. 
% 此外，作者没有考虑他们的对抗性攻击框架的实际部署，而 Nasr 等人。 [4] 做到了。
% - Therefore, there is no practical evaluation such as latency and bandwidth in this paper. 
% 因此，本文没有延迟和带宽等实际评估。
% - It may lead to a gap between ETA with real-world availability.
% 它可能会导致 ETA 与现实世界的可用性之间存在差距。

% 回复
% 我们在实验室搭建了实验场景部署了我们的方法。
% 并且增加延迟和带宽等实际评估。

Thank you for your suggestion to evaluate our proposed approach in a real-world scenario. We have taken your advice into consideration and conducted an evaluation in an actual operational environment.

To create a realistic setup, we established an intrusion detection system within the network of our computer room. The system utilizes machine learning algorithms for intrusion detection. Within this network, we deployed 5 Windows and 5 Linux servers to simulate both normal and malicious communications, with a specific focus on C\&C (Command and Control) communication.

To facilitate attack testing, we captured a dataset comprising 10,000 samples of normal and abnormal network flows using Tshark, a packet analyzer. This dataset will be instrumental in evaluating the accuracy and effectiveness of our intrusion detection system.

By conducting experiments in this real-world environment, we aim to enhance the practical relevance and reliability of our proposed approach.

We sincerely appreciate your valuable suggestion, which has prompted us to incorporate an evaluation in an operational network environment.


==> response2.tex <==
\section{Resubmission and Response}

Dear Editors and Reviewers,

We are grateful for your letter and the insightful comments provided by the reviewers regarding our manuscript, "Explainable and Transferable Adversarial Attack for ML-Based Network Intrusion Detectors." We appreciate the time and effort put into evaluating our work and providing constructive feedback to improve the quality of our paper.

We have carefully considered all the comments and suggestions provided by the reviewers and have made several revisions to the manuscript accordingly. We believe that these changes have substantially improved the clarity and quality of our work.

The feedback we received from the reviewers has been extremely valuable and has helped us to refine and strengthen our research. We appreciate the thoroughness of the review process and the guidance provided, which has helped us to enhance the significance and relevance of our study.

We would like to thank the reviewers and the editorial team for their valuable input, and we hope that our revised manuscript meets with your approval. We look forward to hearing back from you soon.

The main revisions are summarized as follows:

\subsection{Reply to Associate Editor}
Dear Dr. xxx (Associate Editor):
Thank you very much for your patience and great efforts on our manuscript. 
We have seriously considered for a long time and carefully revised our manuscript according to useful comments from you and two reviewers. 
We have carefully considered every comment from you and the two reviewers and revised our manuscript accordingly. 
However, from some of the reviewers’ comments, we realized that there were misunderstandings of our contributions and methods due to our unclear and inaccurate descriptions in the previous manuscript. 
We apologize for that and carefully revised the manuscript (specific revisions will be stated later in the response to the reviewers). 
We hope that the current version of our manuscript can make it easier for reviewers and readers to understand our work. 

\subsection{Reply to Reviewer 1}
\subsubsection{Expanded Feature Scope}
Original: Only discussed time-series statistical features.

Revised: Section 5.1.3 - Added descriptions of both flow-based features (covering flow sequences, timestamps, protocol fields) and packet-based features. Stated these encompass commonly used features in NIDS.

We appreciate the reviewer's suggestion to include a broader range of feature extractors beyond just time-based statistical features. This is an excellent point - relying solely on a narrow set of features may not be sufficient for modern NIDSs.

To address this concern, we have expanded the features used for evaluation to include both flow-based and packet-based features. The flow-based features incorporate flow sequence statistics, size distributions, timestamps, and other time-series characteristics. They also contain some packet header information such as protocol fields. These flow-based features cover the commonly used features in ML-based intrusion detection systems.

In addition, we have also incorporated packet-based features in our experiments. The packet-based features evaluate incremental statistics of packet properties across time windows. Together, the flow-based and packet-based features encompass the core features typically leveraged in current ML-based NIDSs. While other specialty feature extractors exist, the information contained substantially overlaps with our comprehensive feature set.

By expanding the features under consideration, we aim to capture a broader, more representative range of characteristics that are relevant for intrusion detection in modern NIDSs. Overall, we believe the augmented flow-based and packet-based feature set adequately covers the fundamental traits and patterns of network traffic.

\subsubsection{Limited Knowledge Experiments}
Original: Assumed attacker knows all features and data.

Revised: Section 5.3 - Added new experiments with partial knowledge of features and dataset. Results show high attack success with limited knowledge.

We appreciate the reviewer raising an important concern regarding the realism of the threat model's assumption that the attacker possesses full knowledge of the features and data. This is a valuable critique.

In response, we have conducted additional experiments to evaluate attack success under more limited adversary knowledge. Specifically, we consider three scenarios representing partial knowledge:

Limited Feature Knowledge: The attacker only knows a subset of the features used by the model.
Limited Data Knowledge: The attacker only has access to a fraction of the training data.
Cross-Feature Transfer: The attacker evaluates their ability to transfer attacks from one feature set to another.
The results demonstrate that even with such restricted knowledge, the attack can still achieve relatively high success rates. This is because the method is designed to pinpoint and exploit fundamental vulnerabilities in the feature extraction process itself.

Moreover, we would like to clarify that the main focus of our method is on transferability across different model architectures, rather than features or datasets. Under this context, the assumption of partial knowledge of features and data is reasonable.

\subsubsection{Clarified Threat Model and Claims}
Original: Overgeneralized claims about black-box attack applicability.

Revised: Abstract, Introduction, Section 3.2 - Clarified our method only applies to subset of statistical NIDS models. Removed claims about general black-box applicability.

We appreciate the reviewer raising the important concern regarding the feasibility of transfer-based attacks if the target NIDS is a pure black-box system without any commonalities with other NIDS models. This is an insightful critique.

To address this issue, we have focused on two key strategies:

Identifying Non-Robust Features: We target features likely to be non-robust, i.e. vulnerable to attacks due to flaws in the feature extraction itself. By exploiting weaknesses in the input features, we can enable transferability across diverse NIDS models.
Integrated Model with Min-Max Game: We employ an integrated model and min-max game techniques to enhance transferability across models with minimal commonality. This approach facilitates exploring vulnerabilities and attack strategies that could be effective even for pure black-box NIDS.
Furthermore, we demonstrate high attack success under limited knowledge of the model, features, and data. This helps validate the transferability of our approach even absent shared characteristics between the NIDS models.

We sincerely appreciate the reviewer raising this important concern. It pushed us to strengthen the techniques to enable transferability against black-box models. The suggested improvements also help validate our method's capabilities under more challenging and realistic threat conditions. 

I sincerely appreciate you requesting this level of detail in the changes. Please let me know if you would like me to expand or clarify any part of my explanations above. Your feedback is extremely helpful for improving my response specificity.

Reply to Reviewer 2
\subsubsection{Additional Target Models}
Original: Only covered a limited set of classical NIDS models.

Revised: Section 5.1.3 - Added models like MaMPF, FS-Net, AlertNet, DeepNet, IDSNet covering more ML techniques.

We appreciate the reviewer's insightful comments regarding the representativeness of the target NIDS models used in our study. This is an excellent critique pointing out an opportunity for improvement.

Acting on the reviewer's feedback, we have expanded the set of target models to better reflect the state-of-the-art and diversity of techniques used in modern NIDSs. Specifically, we have incorporated the following additional models into our experiments:

MaMPF
FS-Net
AlertNet
DeepNet
IDSNet
These models cover a broader range of relevant machine learning approaches and are widely adopted in the field. By expanding the diversity of target NIDS models under examination, we aim to strengthen the generalizability and real-world effectiveness of our proposed attack method.

We also appreciate the reviewer thoughtfully suggesting the inclusion of more sequence-based models such as RNNs and Markov models. However, the primary focus of our work is evaluating the cross-model transferability of attacks between different architectures. The time-series models included in our study provide a strong basis for comprehensively assessing transferability across a varied set of NIDS techniques.

\subsubsection{Incorporated Highly Relevant Work}
Original: Missed important prior work on blind perturbations.

Revised: Section 2.2.3 - Incorporated the work by Nasr et al. on GAN blind perturbations. Implemented their method as a baseline.

Thank you for pointing out that we missed citing the important related work by Nasr et al., "Real-Time Robust Malicious Traffic Detection with Blind Adversarial Perturbations", published in Usenix 2021. This is indeed a crucial paper we should have referenced.

To address this, we have added Nasr et al.'s work to the Related Work section and provided an overview of their approach using generative adversarial networks (GANs) to generate blinding adversarial perturbations that fool deep neural network-based traffic analysis systems. We have carefully studied their paper to ensure we accurately reflect its contributions in our revised manuscript.

We believe our work and theirs are complementary, as we both aim to improve the robustness of ML-based network intrusion detection systems against adversarial attacks. To enable comparison, we have also implemented their GAN-based adversarial attack as a baseline in our experiments.

We sincerely appreciate you catching this important omission. Adding this highly relevant work helps improve the completeness of our literature review and gives readers a more comprehensive view of the state-of-the-art.

\subsubsection{Traffic Constraint Details}
Original: Lacked details on satisfying traffic constraints.

Revised: Section 4.5.2 - Provided more specifics on transforming adversarial examples to pass TCP validation.

Thank you for the feedback regarding the lack of details on satisfying traffic space constraints. This is an important aspect we should explain more clearly.

Acting on your suggestion, we have expanded the manuscript to provide a more thorough description of how we transform adversarial examples to comply with traffic constraints.

Specifically, we have added details on the traffic spatial transformations performed to ensure the modified packets conform to TCP finite state machine verification and other relevant protocol requirements. This includes constraints on sequence numbers, flags, checksums, and other packet attributes that must be consistent for packets to be valid.

By outlining the specific steps taken to satisfy protocol correctness and preserve attack semantics, we aim to give readers a better understanding of how the manipulated packets can realistically be leveraged to evade NIDS in practice.

We appreciate you highlighting this opportunity to improve the manuscript's clarity. Please let us know if you have any other recommendations on how we can better explain the traffic constraints and modifications to enable practical deployment.

\subsubsection{Real-World Experiments}
Original: No evaluation in live settings.

Revised: Section 5.7 - Set up testbed on university network. Evaluated performance metrics like latency and bandwidth.

Thank you for the insightful suggestion to evaluate our approach in a real-world deployment. We fully agree on the importance of testing performance in live settings.

Following your advice, we have set up an experimental intrusion detection system within our university's computer network. The system uses machine learning algorithms for detection.

To create a realistic environment, we deployed 5 Windows and 5 Linux servers to simulate normal traffic and C2 malicious communications. Using Tshark, we captured a dataset of 10,000 network flow samples containing both normal and attack traffic.

By testing our attack against the live IDS using real-world data, we can better validate the practical applicability and effectiveness of our approach. The experiments also allow us to measure relevant performance metrics like latency, bandwidth overhead, and evasion success rates.

We sincerely appreciate you recommending this valuable experiment. Conducting evaluations on an operational network with live data significantly enhances the real-world relevance of our results.

Please let me know if I can elaborate or clarify any part of my response. I appreciate you asking me to directly cite the revised sections, as it helps me articulate the changes precisely. Your feedback is extremely valuable.
